Distribution Learning for Molecular Regression

Using "soft" targets to improve model performance has been shown to be effective in classification settings, but the usage of soft targets for regression is a much less studied topic in machine learning. The existing literature on the usage of soft targets for regression fails to properly assess the method's limitations, and empirical evaluation is quite limited. In this work, we assess the strengths and drawbacks of existing methods when applied to molecular property regression tasks. Our assessment outlines key biases present in existing methods and proposes methods to address them, evaluated through careful ablation studies. We leverage these insights to propose Distributional Mixture of Experts (DMoE): A model-independent, and data-independent method for regression which trains a model to predict probability distributions of its targets. Our proposed loss function combines the cross entropy between predicted and target distributions and the L1 distance between their expected values to produce a loss function that is robust to the outlined biases. We evaluate the performance of DMoE on different molecular property prediction datasets -- Open Catalyst (OC20), MD17, and QM9 -- across different backbone model architectures -- SchNet, GemNet, and Graphormer. Our results demonstrate that the proposed method is a promising alternative to classical regression for molecular property prediction tasks, showing improvements over baselines on all datasets and architectures.

==> tables/bin-dist-ablation.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table}[!htp]\centering
    \caption{Validation results for running GemNet-dT+Pos+DMoE on the ID split of the OC20 IS2RE dataset, varying the bin distribution, number of histograms, and number of bins}\label{tab:bindist-ablation}
    \scriptsize
    \begin{tabular}{lrrrr}\toprule
                                  & \(N_{\text{histogram}} \text{ x } N_{\text{bins}}\) & Energy MAE     & EWT            \\\midrule
        \multirow{3}{*}{Uniform}  & 32x2048                                             & 0.467          & 6.5\%
        \\
                                  & 64x1024                                             & \textbf{0.464} & \textbf{7.2}\%
        \\
                                  & 256x256                                             & 0.466          & 7.1\%
        \\
        \hline
        \multirow{3}{*}{Gaussian} & 32x2048                                             & \textbf{0.454} & \textbf{8.3}\%
        \\
                                  & 64x1024                                             & 0.455          & 7.9\%
        \\
                                  & 256x256                                             & 0.459          & 7.3\%
        \\
        \bottomrule
    \end{tabular}
\end{table}


==> tables/gemnet-alpha-beta-ablation.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table}[!htp]
    \centering
    \caption{The impact of different HL and DL coefficients on the performance of the GemNet+Pos model on the ID split of OC20}\label{tab:alpha-beta-ablation}
    \scriptsize
    \begin{tabular}{lrrrr}\toprule
        \(\alpha_{HL}\)               & \(\alpha_{DL}\) & E-MAE & EWT            \\\midrule
        1.00                          & 0.00            & 0.455 & \textbf{8.3\%} \\
        0.90                          & 0.10            & 0.457 & 8.0\%          \\
        0.75                          & 0.25            & 0.459 & 8.1\%          \\
        0.50                          & 0.50            & 0.457 & 8.1\%          \\
        0.25                          & 0.75            & 0.462 & 7.9\%          \\
        0.10                          & 0.90            & 0.473 & 7.3\%          \\
        0.00                          & 1.00            & 2.253 & 0.8\%          \\
        \multicolumn{2}{c}{Scheduled} & \textbf{0.450}  & 7.8\%                  \\
        \bottomrule
    \end{tabular}
\end{table}


==> tables/qm9.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table}[!htp]\centering
    \caption{Validation scores for the MXMNet backbone model on the QM9 dataset}\label{tab:qm9}
    \scriptsize
    \begin{tabular}{lrr|rrr}\toprule
                              & \multicolumn{2}{c}{Baseline} & \multicolumn{2}{c}{\methodacronym{}}                                     \\\cmidrule{2-5}
                              & MAE                          & WT                                   & MAE             & WT              \\\midrule
        \(\mu\) (D)           & 0.0444                       & 56.9\%                               & \textbf{0.0397} & \textbf{60.9\%} \\
        \(a\) (\(a^3_{0}\))   & \textbf{0.0624}              & \textbf{95.9\%}                      & 0.0716          & 95.1\%          \\
        \(e_{HOMO}\) (eV)     & 0.0290                       & 26.5\%                               & \textbf{0.0275} & \textbf{33.1\%} \\
        \(e_{LUMO}\) (eV)     & 0.0227                       & \textbf{40.2\%}                      & \textbf{0.0225} & 39.9\%          \\
        \(\Delta e\) (eV)     & 0.0456                       & 29.8\%                               & \textbf{0.0414} & \textbf{36.4\%} \\
        \(R^2\) (\(a^2_{0}\)) & 1.3034                       & 93.9\%                               & \textbf{0.9813} & \textbf{95.9\%} \\
        \(ZPVE\) (eV)         & 0.0015                       & 99.1\%                               & \textbf{0.0014} & \textbf{99.5\%} \\
        \(U_{0}\) (eV)        & \textbf{0.0226}              & \textbf{98.9\%}                      & 0.0236          & \textbf{98.9\%} \\
        \(U\) (eV)            & \textbf{0.0143}              & \textbf{99.7\%}                      & 0.0235          & 98.9\%          \\
        \(H\) (eV)            & \textbf{0.0144}              & \textbf{99.6\%}                      & 0.0228          & 99.0\%          \\
        \(G\) (eV)            & \textbf{0.0138}              & \textbf{99.6\%}                      & 0.0223          & 98.7\%          \\
        \(c_{v}\) (cal/mol.K) & \textbf{0.0253}              & \textbf{82.7\%}                      & 0.0272          & 80.5\%          \\
        \bottomrule
    \end{tabular}
\end{table}


==> tables/uncertainty.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table}[!htp]\centering
    \caption{Uncertainty metrics for GemNet-dT evaluated on the OC20 ID validation split}\label{tab:uncertainty}
    \scriptsize
    \begin{tabular}{lrrrr}\toprule
                                            & MACE            & RMSCE           & MA              \\\midrule
        Ensemble                            & 0.2752          & 0.3119          & 0.2780          \\
        Ensemble + IR Recal                 & 0.0237          & 0.0334          & 0.0240          \\
        \methodacronym{}-Entropy            & 0.0427          & 0.0668          & 0.0431          \\
        \methodacronym{}-Entropy + IR Recal & 0.0116          & 0.0303          & 0.0117          \\
        \methodacronym{}-KL                 & 0.0542          & 0.0664          & 0.0547          \\
        \methodacronym{}-KL + IR Recal      & \textbf{0.0057} & \textbf{0.0165} & \textbf{0.0057} \\
        \bottomrule
    \end{tabular}
\end{table}

